Learning with Capsules: A Survey

Capsule networks were proposed as an alternative approach to Convolutional Neural Networks (CNNs) for learning object-centric representations, which can be leveraged for improved generalization and sample complexity. Unlike CNNs, capsule networks are designed to explicitly model part-whole hierarchical relationships by using groups of neurons to encode visual entities, and learn the relationships between those entities. Promising early results achieved by capsule networks have motivated the deep learning community to continue trying to improve their performance and scalability across several application areas. However, a major hurdle for capsule network research has been the lack of a reliable point of reference for understanding their foundational ideas and motivations. The aim of this survey is to provide a comprehensive overview of the capsule network research landscape, which will serve as a valuable resource for the community going forward. To that end, we start with an introduction to the fundamental concepts and motivations behind capsule networks, such as equivariant inference in computer vision. We then cover the technical advances in the capsule routing mechanisms and the various formulations of capsule networks, e.g. generative and geometric. Additionally, we provide a detailed explanation of how capsule networks relate to the popular attention mechanism in Transformers, and highlight non-trivial conceptual similarities between them in the context of representation learning. Afterwards, we explore the extensive applications of capsule networks in computer vision, video and motion, graph representation learning, natural language processing, medical imaging and many others. To conclude, we provide an in-depth discussion regarding the main hurdles in capsule network research, and highlight promising research directions for future work.

==> sections/10_medical_imaging.tex <==
\section{Medical Imaging}

Another field that Capsules have been applied fairly extensively to is that of medical imaging \cite{afshar2019capsule, zhang2019cervical, wang2020multikernel, gaddipati2019glaucoma, liu2019wbcaps}. This is largely in part due to a Capsule Networks ability to generalise to new variations of the learnt classes in unseen data which were not captured in the training data. Additionally this property is achieved after being trained on the small amount of data which is typical for medical datasets due to the expertise required in labelling.

SegCaps \cite{lalonde2018capsules} replaces the convolutional blocks of a U-Net \cite{ronneberger2015unet} with convolutional capsule blocks and modifies dynamic routing to be locally connected by only routing capsules in layer L to parent capsules in layer L+1 within a $k_h \times k_w$ kernel to semantically segment 2D slices of computed tomography (CT) scans showing irregular lesions and nodules. The modified Dynamic Routing alogrithm is shown below. This method achieved state of the art Dice Coefficient on the LUNA16 dataset with 98.479\% accuracy while also reducing the parameters by 95.4\%. 
%
Again, applied to detection of nodules in CT scans, Fast CapsNet \cite{mobiny2018fast} modified dynamic routing CapsNet \cite{sabour2017dynamic} in order to scale to 3D data. Their contributions are to add a constraint which allows only one Capsule per pixel location in the Primary Capsules. By doing this they reduce the computational overhead of routing by agreement by 32x resulting in a 3x overall increase of network training per epoch while retaining approximately the same accuracy as base CapsNets on 2D images which were slices of a 3D volume of the full CT scan. While this change may be small for 2D data, when they attempted to apply base CapsNets to 3D scans the network was unable to be trained stably whilst their modified CapsNet was able to achieve better accuracy on 3D than 2D data. Additionally they replace the fully connected layers in the decoder section of the CapsNet with deconvolutional layers. Overall they achieve 91.84\% accuracy which is greater than the 91.05\% accuracy provided by the best CNN based architectures and greatly improved upon the 73.65\% provided by non deep learning approaches. 

In the realm of Brain Tumour classification, CNNs have been shown to fail to utilise the spatial relationships between brain perturbations which causes misdiagnosis of tumours. As a result of this, the authors in \cite{afshar2019capsule} propose using a locally routed Capsule Network similar to \cite{mobiny2018fast}. Additionally, rough boundaries of where the tumours are located are given to the network to ensure that it ignores irrelevant areas of the image. When trained with the entire image without rough tumour boundaries, the network achieves 78\% accuracy on their dataset of MRI scans. This is then improved to 90.89\% when additionally given the rough tumour boundaries, slightly improving upon the state of the art CNNs which are able to achieve 88.33\% accuracy when given the rough tumour boundaries.

Building upon their previous work in \cite{lalonde2018capsules}, \cite{lalonde2021capsules} extends their work to five new datasets as well as introducing the condition that child capsules are only routed within a spatially located window. This change allows their network to scale to images of 512x512 size while remaining at around 1.5 million parameters. For reference a standard dynamically routed capsule network would require approximately 2 quadrillion parameters to scale to images of this size. Again, their method is able to outperform state of the art networks in five datasets DICE coefficient and outperforms in four of the five datasets in Hausdorff Distance score. Additionally it should be noted that their method has a significantly lower standard deviation between runs on different random seeds.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{images/SegCaps_architecture.png}
    \caption{The architecture for SegCaps, which uses Capsule Networks in a u-net like architecture combining the information learnt at different levels of downscaling via Capsule Network convolutional layers. The deconvolutional Capsule layer is also used before a final convolutional Capsule layer. Figure from ~\cite{lalonde2018capsules}.}
    \label{fig:covid-caps}
\end{figure}

Covid-19 created a demand for fast and accurate diagnosis of patients. As a result multiple deep learning techniques were tested upon CT scan and x-rays of lungs. Motivated by Capsules Networks ability to achieve strong results with low amounts of data, COVID-CAPS \cite{AFSHAR2020638} was devised. Utilising a standard dynamic routing \cite{sabour2017dynamic} architecture to classify either positive or negative for Covid-19, COVID-CAPS is able to achieve an accuracy of 95.7\%. When pre-trained using a large dataset of other x-ray images, COVID-CAPS is able to achieve 98.3\% accuracy.

Similarly, \cite{li2021mha} propose MHA-CoroCapsule a novel capsule architecture which builds upon the dynamic routing capsules \cite{sabour2017dynamic} by replacing the dynamic routing element with a non iterative multi-head attention routing process. By using a dataset of under 300 lung x-rays of Covid-19 patients they were able to achieve nearly state of the art results of 97.28\% accuracy compared to 98.30\% achieved by COVID-CAPS \cite{AFSHAR2020638}, however COVID-CAPS is pre-trained on over 100 thousand images of other lung diseases compared to the 1 thousand total images used in MHA-CoroCapsules.

==> sections/9_nlp.tex <==
\section{Natural Language Processing}

Capsule networks have gained popularity in the field of natural language processing due to their ability to model part-whole relationships. Here, the sentence parts are individual words and the routing procedure learns the spatial and semantic relationships between the sentences components. Capsule-based architectures have been applied to a variety of natural language tasks including text classification, relation extraction, search personalization, and recommender systems.

\textbf{Text Classification} Text classification spans several tasks including sentiment classification, question categorisation, news categorisation, and intent detection. Yang \etal \cite{yang2018investigating} first explored the use of capsule networks in natural language processing for the problem of text classification. Here, the dynamic routing algorithm \cite{sabour2017dynamic} is augmented to deal with noisy capsules in three ways: the addition of orphan (i.e. background) categories, the use of leaky-softmax instead of the standard softmax operation to obtain the routing coefficients, and the multiplication of routing coefficients by the probability of existence of child capsules (denoted coefficient amendment). This work shows that capsule network can achieve strong performance across 6 datasets when compared with standard neural network methods like CNNs and LSTMs. Kim \etal \cite{kim2020text} also propose a capsule network for text classification. To circumvent the need for max-pooling the text sequence, this work makes use of an ELU-gate unit that does not lose spatial information. Following the gate unit, the primary capsules are generated and passed through a ``static routing" procedure which consists of a single forward pass of the dynamic routing algorithm. Another work \cite{zhao2019towards} attempts to adapt capsule networks to be more successfully applied to NLP applications. First, a capsule compression operation is performed which merges similar capsules to reduce the number of primary capsules. Then, for routing an adaptive optimizer is introduced which allows for a variable number of routing iterations for a given sample. Lastly, for final classification a partial routing procedure allows for a reduced number of output capsules to be produced and leading to a large reduction on computational cost.

\begin{figure}[t]
        \centering
        \includegraphics[width=\columnwidth]{images/nlpcaps.png}
        \caption{Architecture of a Capsule Network for text classification. The adjusted local spatial routing between the Primary Capsules and the Convolutional Capsules is shown in detail. Figure from ~\cite{yang2018investigating}.}
        \label{fig:nlpcaps}
\end{figure}

Another work \cite{xia2018zero} utilizes capsule networks for the task of zero-shot user intent detection. The proposed capsule network can detect intents unseen at training time by modifying the dynamic routing algorithm with self-attention and allowing for the generation of capsules for emerging intents (\ie intents not used during training). Furthermore, analysis of the routing coefficients illustrate the capsule networks' ability to model the relationships between parts (words) and their corresponding whole (intents). Chen \etal \cite{chen2019transfer} propose a Transfer Capsule Network (TransCap) for the problem of aspect-level sentiment classification (\ie  classifying the sentiment of a specific aspect occurring in a sentence). Given a sentence and the given aspect, TransCap generates a set of feature capsules from the input words and then performs ``aspect routing" which gates the sentence (context) capsules using the aspect features to generate semantic capsules (SemanCaps). These SemanCaps are then passed through the dynamic routing algorithm to obtain the final classification capsule layer. Capsules have also been applied to the task of slot filling and intent detection \cite{zhang2018joint}. For a given sentence, this task involves a two-step classification problem: first assigning words to a specific slot class (\eg \textit{artist}, \textit{playlist}, \textit{movie\_type}) and then classifying the intent of the overall query (\eg \textit{change\_playlist}, \textit{play\_music}). Zhang \etal \cite{zhang2018joint} propose a capsule network which generate a capsule for each word in the sentence and applies dynamic routing to create a set of slot capsules. The routing coefficients represent the assignment of each word in the sentence to a slot class. Then, another routing operation is used to obtain the final intent capsules and the final intent classification.

\textbf{Relation Extraction} Relation extraction is a problem involving finding the relationships between different entities (\ie words) within a sentence. Zhang \etal \cite{zhang2018attention} illustrate capsule networks' ability to learn these relationships. The proposed capsule network makes use of a bi-directional LSTM to generate the initial capsule layer. Then, dynamic routing with coefficient amendment is used to generate a set of parent capsules, whose activations are the probabilities of different relations. The entities by which these relations are represented are determined through another pretrained method \cite{han2018openke}. Another work \cite{zhang2019multi} proposes the architecture Att-CapNet which also uses a bi-LSTM to generate the initial capsule layer. Here, however, the hidden states of the recurrent model are also used in the generation of attention coefficients for improved capsule routing. 

\textbf{Search Personalization and Recommendation Systems} Capsule networks have been applied to knowledge graph completion for the task of user search personalization \cite{vu2019capsule}. For this problem, the goal is to generate a rating for a tuple (\textit{query}, \textit{user}, \textit{document}), such that the output document is personalized for a given user's query. Vu \etal use a capsule-based approach which first encodes all elements of the tuple into vectors, and use convolution operations to generate a set of primary capsules. Then, the dynamic routing algorithm is used to generate a single two-dimensional capsule whose magnitude determines the score for the given tuple. A higher score denotes that there was agreement between the input capsules, leading to a higher ranking for the document when given the user's query. Capsules have also been used in recommendation systems. Given a set of reviews generated by a user and reviews for various items, recommendation systems attempt to suggest which items the user would like the most. Li \etal \cite{li2019capsule} present a capsule-based architecture, which takes embeddings for user and item reviews, and generates a set of positive and negative capsules to represent the sentiment of various aspects of the reviews. Then, a routing by bi-agreement algorithm is proposed which attempts to find agreement not only between different capsules, but also within dimensions of the same capsules (both inter-capsule and intra-capsule agreement). From the output of the routing algorithm, a recommendation score (\ie rating) is generated for the given item.

\textbf{Language and Vision} Several applications require the use of both textual and visual data. Capsules networks have shown promise in these multi-modal tasks. One such problem is that of visual question answering where a natural language question is given for an image, and the goal is to select a multiple choice answer or generate natural language answer. One of the first capsule-based approaches for this task is \cite{zhou2019dynamic}. Here, routing-by-agreement is used as an attention mechanism between the visual and textual features to improved learned representations.  Urooj \etal \cite{urooj2021found} propose a capsule framework for visual question answering grounding systems. This work shows that including capsules with EM-routing \cite{hinton2018matrix} in the generation of visual features leads to drastic improvement in grounding accuracy; the capsule architecture uses relevant visual information in intermediate reasoning steps. Recently, Cao \etal \cite{cao2021linguistically} present a routing algorithm that adjusts the capsule routing weights based on the parse tree generated from the given question. The proposed linguistically routed capsule network is shown to achieve strong visual questioning answering performance, even on out-of-distribution data. Capsule networks have also been applied to multimodal machine translation \cite{lin2020dynamic}. The goal of this problem is to improve the translation a natural language sentence with visual features. Lin \etal \cite{lin2020dynamic} propose a context-guided dynamic routing procedure to update the routing coefficients between visual capsules using cross-modal correlations. They show that this context-guided routing outperforms the standard attention and dynamic routing mechanisms when applied to their approach.


\iffalse

Text Classification

1. Investigating capsule networks with dynamic routing for text classification (EMNLP2018) - yang2018investigating
- first paper with caps and NLP
- Augments Sabour etal. routing to deal with noisy capsules in 3 ways: "orphan category" (i.e. additional background capsules), leaky-softmax instead of regular in obtaining routing coefficients, and coefficient amendment (i.e. multiplying routing coefficient by probability of existence of child capsules). 
- Evaluate on 6 datasets spanning tasks like sentiment classification, question categorization, news categorization
- Compare with standard neural network methods like CNNs and LSTMs

2. Zero-shot User Intent Detection via Capsule Neural Networks (EMNLP2018) - xia2018zero
- performs intent detection in a zero-shot manner
- augment routing algorithm with self-attention, and allow for the generation of capsules for emerging intents (i.e. classes unseen during training)
- they show that the routing coefficients focus on specific words pertaining to the given intent (i.e. correctly learns the parts (words) which correspond to the whole (intent)

Relation Extraction (i.e. predicts relations between different entities in a sentence)

1. Attention-Based Capsule Networks with Dynamic Routing for Relation Extraction (EMNLP2018) - zhang2018attention
- uses bi-lstm to obtain primary capsules
- uses coefficient amendment from zhao etal.
- parent capsule activations are the probabilities of different relations, and the entities which these relations are represented by are determined by using a another pretrained method.

2. Multi-labeled Relation Extraction with Attentive Capsule Network (AAAI2019) - zhang2019multi
- bi-lstm used to obtain primary capsules and for generating attention coefficients to augment the routing method


 
 

\fi
